Safety-Aware Task Composition for Discrete and Continuous Reinforcement Learning

Compositionality is a critical aspect of scalable system design. Reinforcement learning (RL) has recently shown substantial success in task learning, but has only recently begun to truly leverage composition. In this paper, we focus on Boolean composition of learned tasks as opposed to functional or sequential composition. Existing Boolean composition for RL focuses on reaching a satisfying absorbing state in environments with discrete action spaces, but does not support composable safety (i.e., avoidance) constraints. We advance the state of the art in Boolean composition of learned tasks with three contributions: i) introduce two distinct notions of safety in this framework; ii) show how to enforce either safety semantics, prove correctness (under some assumptions), and analyze the trade-offs between the two safety notions; and iii) extend Boolean composition from discrete action spaces to continuous action spaces. We demonstrate these techniques using modified versions of value iteration in a grid world, Deep Q-Network (DQN) in a grid world with image observations, and Twin Delayed DDPG (TD3) in a continuous-observation and continuous-action Bullet physics environment. We believe that these contributions advance the theory of safe reinforcement learning by allowing zero-shot composition of policies satisfying safety properties.

==> sections/tl-comp.tex <==
\section{Temporal Logic Task Composition}

\begin{itemize}
    \item Learn the positive and negative versions of each task with penalties
    \item Assume we can build an underapproximation of the environment (either done at training time or runtime)
    \item Create a product between underapproximate MDP and the LTL B{\"u}chi automata
    \item Run traditional planning over the product automaton (Djikstra's etc...)
    \item Execute the plan via Boolean compositions
\end{itemize}
